Empirical Bayes Predictive Density Estimation under Covariate Shift in Large Imbalanced Linear Mixed Models

We study empirical Bayes (EB) predictive density estimation in linear mixed models (LMMs) with large number of units, which induce a high dimensional random effects space. Focusing on Kullback Leibler (KL) risk minimization, we develop a calibration framework to optimally tune predictive densities derived from on a broad class of flexible priors. Our proposed method addresses two key challenges in predictive inference: (a) severe data scarcity leading to highly imbalanced designs, in which replicates are available for only a small subset of units; and (b) distributional shifts in future covariates. To estimate predictive KL risk in LMMs, we use a data-fission approach that leverages exchangeability in the covariate distribution. We establish convergence rates for our proposed risk estimators and show how their efficiency deteriorates as data scarcity increases. Our results imply the decision-theoretic optimality of the proposed EB predictive density estimator. The theoretical development relies on a novel probabilistic analysis of the interaction between data fission, sample reuse, and the predictive heat-equation representation of George et al. (2006), which expresses predictive KL risk through expected log-marginals. Extensive simulation studies demonstrate strong predictive performance and robustness of the proposed approach across diverse regimes with varying degrees of data scarcity and covariate shift.

==> append.tex <==



\noindent \textbf{Proof of Theorem~\ref{thm.risk.conv}.}
The proof of the theorem involves the following steps. We need to prove:\\
\textbf{Step 1.} $\hat R_{1,n}^{\,g}- R_{1,n}^{\,g}=O_p({(\log\log n)}/\sqrt{n})$.\\
\textbf{Step 2.} $\hat R_{2,n}^{\,g}(h) -  \hat R_{2,n}^{\,g}=O_p({(\log\log n)}(D_n/\sqrt{n})$.\\
\textbf{Step 3.} $\hat R_{2,n}^{\,g}(h) -  R_{2,n}^{\,g}=O_p({(\log\log n)}D_{n}/\sqrt{n})$.

\noindent Then, we calculate the asymptotic rate of $D_n$.

\noindent \textbf{Proof of Step 1.} 
%The proof follows in the similar line to the proof of Theorem~4.1 in \citet{george2021optimal}. 
%First note that, Assumption A4 along with Assumption 1 implies: 
%$$\frac{1}{n} \sum_{i=1}^n \text{Var}(\log m^g(v_i\dot X_i;u_i,v_i))< \infty$$
We begin with bounding 
\begin{align*}
M_{i}^{2}&:=\mathrm{Var}\left[
\left(\sum_{i=1}\tilde{K}_{i}\right)^{-1}
\sum_{k=1}^{\tilde{K}_{i}}
\{\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)\}
\right].
\end{align*}
By applying Jensen's inequality to the function $y\to y^{2}$, we have
\begin{align*}
M_{i}^{2}
&\le 
\left(\sum_{i=1}^{n}\tilde{K}_{i}\right)^{-2}
\mathbb{E}\left[
\left\{
\sum_{k=1}^{\tilde{K}_{i}}
\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)
\right\}^{2}
\right]\\
&\le
\left(\sum_{i=1}^{n}\tilde{K}_{i}\right)^{-2}
\tilde{K}_{i}\sum_{k=1}^{\tilde{K}_{i}}
\mathbb{E}\left[
\left(
\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)
\right)^{2}
\right].
\end{align*}
Then, consider bounding 
$\mathbb{E}[
(
\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)
)^{2}$.
Observe 
\[
m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)
=\int \phi(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i}\gamma,u_{i}^{-1}v_{ik}\hat \sigma)g(\gamma)d\gamma
\le
1/\{\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma)\},
\]
and so, we can upper bound $\mathbb{E}[(\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma))^{2}$ by
\begin{align*}
&
\mathbb{E}\left[
\left(
\log \frac{m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)}{
(\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma))^{-1}
}
+\log \frac{1}{\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma)}
\right)^{2}
\right]\\
&\le
2
\mathbb{E}\left[
\left(
\log \frac{m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)}{
(\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma))^{-1}
}
\right)^{2}
\right]
+2(\log \{\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma)
\}
)^{2}.
\end{align*}
By Jensen's inequality the above is again bounded by
\begin{align*}
2\mathbb{E}\bigg\{\mathbb{E}_{\gamma\sim g}
\left(
\log \frac{\phi(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i}\gamma,u_{i}^{-1}v_{ik}\hat \sigma)}{
(\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma)^{-1})
}
\right)^{2}\bigg\}
+2(\log \{\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma)
\}
)^{2}.
\end{align*}
Next, by using the inequalities $(a+b)^{2} \le 2a^{2} +2b^{2}$ and $(a+b)^{4}\le 53(a^{4}+b^{4})$,
we finally bound $\mathbb{E}[(\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma))^{2}$ by
\begin{align*}
&4\mathbb{E}\bigg\{\mathbb{E}_{\gamma\sim g}
\left[
\frac{(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma)-u_{i}\gamma)^{2}}{2(u_{i}^{-1}v_{ik}\hat \sigma)^{2}}
\right]^{2}\bigg\}
+
4(\log \{\sqrt{2\pi}(u_{i}^{-1}v_{ik}\hat \sigma)
\}
)^{2}\\
&\le
c\left(
\frac{u_{i}^{4}}{\hat \sigma^{4}}
\mathbb{E}
\left[Z_i(\hat{\bm{\beta}},\hat \sigma)^{4}\right]
+
\frac{u_{i}^{4}}{v_{ik}^{4}\hat \sigma^{4}}
\mathbb{E}_{\gamma\sim g}\left[
\gamma^{4}
\right]
\right)
+(\log 2\pi)^{2} + 4\{\log (u_{i}^{-1}v_{ik}\hat \sigma)\}^{2},
\end{align*}
where, $c$ is an absolute constants (specifically, say, $500$). 
Substituting $\mathbb{E}[Z_i(\hat{\bm{\beta}},\hat \sigma)]=\mathbb{E}_{\gamma\sim g^{*}}\mathbb{E}_{Z_i\mid \gamma}[Z_i(\hat{\bm{\beta}},\hat \sigma)]$ where the true distribution of $\gamma$ is denoted by $g^{*}$, 
we further simplify the upper bound on $\mathbb{E}[
(\log m^{g}(v_{ik}Z_i(\hat{\bm{\beta}},\hat \sigma);u_{i},v_{ik},\hat \sigma)
)^{2}$ as
\begin{align*}
 c'\left(
\frac{u_{i}^{4}}{\hat \sigma^{4}}
\mathbb{E}_{\gamma\sim g^{*}}[\gamma^{4}]
+3+\frac{u_{i}^{4}}{v_{ik}^{4}\hat \sigma^{4}}
\mathbb{E}_{\gamma\sim g}\left[
\gamma^{4}
\right]
\right)+(\log 2\pi)^{2} + 4\{\log (u_{i}^{-1}v_{ik}\hat \sigma)\}^{2},
\end{align*}
where $c'$ is an absolute constant.
Thus, we get
\begin{align*}
M_{i}^{2}
&\le \left(\sum_{i=1}^{n}\tilde{K}_{i}\right)^{-2}
\left(\tilde{K}_{i}^{2}c''+ \tilde{K}_{i}^{2}\frac{u_{i}^{4}}{\hat \sigma^{4}}\mathbb{E}_{\gamma\sim g^*}[\gamma^{4}]
+
\tilde{K}_{i}\frac{u_{i}^{4}}{\hat \sigma^{4}}
\mathbb{E}_{\gamma\sim g}[\gamma^{4}]
\sum_{k=1}^{\tilde{K}_{i}}
v_{ik}^{-4}
\right)\\
&=
\left(\sum_{i=1}^{n}\tilde{K}_{i}\right)^{-2}\tilde{K}_{i}^{2}
\left(c''+ \max_{i}(u_{i}^{-1}\hat \sigma)^{-4}
\mathbb{E}_{\gamma\sim g^{*}}[\gamma^{4}]
+
\max_{i,k}(u_{i}^{-1}v_{ik}\hat \sigma)^{-4}
\mathbb{E}_{\gamma\sim g}[\gamma^{4}]
\right)\\
&=
\left(\sum_{i=1}^{n}\tilde{K}_{i}\right)^{-2}\tilde{K}_{i}^{2}
\left(c''+ \max_{i}(u_{i}^{-1} \sigma)^{-4}
\mathbb{E}_{\gamma\sim g^{*}}[\gamma^{4}]
+
\max_{i,k}(u_{i}^{-1}v_{ik} \sigma)^{-4}
\mathbb{E}_{\gamma\sim g}[\gamma^{4}] + O_p(n^{-\alpha})
\right)
\end{align*}
% where $c''$ is an absolute constant plus 
% $4\max_{i,k}{(\log u_{i}^{-1}v_{ik}\sigma_{i})^{2}}$.
by assumption (A1) and (A2). So, we finally get
\[
\sum_{i=1}^{n}M_{i}^{2}\le n^{-1}
c'''
\quad \text{with a constant $c'''$ independent from $n$},
\]
which completes Step 1.

\noindent \textbf{Proof of Step 2.} 
Hereafter,
without any loss of generality we assume $\Kf_i=1$ for all $i=1,\ldots,n$. 
We denote $S_{ik}$ as $S_i$ as  $\Kf_i=1$. We recall the proposed estimator for $R_{2,n}$
\begin{align}\label{eq:hat.R2}
\hat R_{2,n}^g(h)=\bigg(\sum_{i=1}^n \Kf_i\bigg)^{-1}\sum_{i=1}^n \sum_{k=1}^{\Kf_i} \hat r_{ik}(g) \,\,1\{(i,k) \in \mathcal{I}(h)\}~.
\end{align}
% Also, without loss of generality we can assume: $0<u_1^2<u_2^2<\ldots<u_n^2$. 
% This implies:\\
% (a) $|S_i|\leq i-1$ for $i=1,\ldots,n$; \\
% (b) $|S_i|$ is monotonically non-decreasing in $i$;\\
% (c) if $j \in S_i$ then $k \in S_i$ for all $k <j$. \\
% Thus, we will using $\phatu$ for $i=1$ and for all other $i$ such that $|S_i|=0$.

Define $s_i=|S_i|$, and recall, the set of improved coordinates, $\mathcal{I}_{F,n}$. We use $\hat r_{ik}$ for $i\in \mathcal{I}_{F,n}$.

Note that:
\begin{align*}
\hat R_{2,n}^g(h) &= \bigg(\sum_{i=1}^n \Kf_i\bigg)^{-1}\sum_{i=1}^n \hat r_{ik}(g)\, 1\{i \in \mathcal{I}_{F,n}\}\\ &= \bigg(\sum_{i=1}^n \Kf_i\bigg)^{-1}\sum_{i \in \mathcal{I}_{F,n}} s_i^{-1} \sum_{j=1}^{n}\ex_{\gamma_j}\big\{\log \tilde m^g(\hat W_{ikj};u_i,v_{ik}, \hat \sigma)\big\}\cdot1\{j \in S_i\}
% &=n^{-1}\sum_{j=1}^{n-1}\sum_{i=j+1}^n s_i^{-1} \ex_{\gamma_j}\big\{\log q^g(\dot T_{ij};u_i,v_{i})\big\}\cdot 1\{j \in S_i\}.
\end{align*}
Similarly, we have:
\begin{align}\label{a.1}
\hat R_{2,n}^{\,g}= \bigg(\sum_{i=1}^n \Kf_i\bigg)^{-1}\sum_{i \in \mathcal{I}_{F,n}}\sum_{j=1}^n s_i^{-1} \ex_{\zeta}\big\{\log \tilde m^g(\hat W_{ikj}(\zeta);u_i,v_{ik},\hat \sigma)\big\}\cdot1\{j \in S_i\}
\end{align}
It is easy to see that $\hat R_{2,n}^{\,g}$ is an unbiased estimate of $R_{2,n}^g(h)$. We next want to calculate its variance. For that purpose, we represent the terms in the right side of \eqref{a.1} as functions of $Z_j(\hat \beta, \hat \sigma)$ for $j=1,\ldots,n$ and apply the following upper bound
$$ \text{Var}\left(\hat R_{2,n}^{\,g}\right) \leq \bigg(\sum_{i=1}^n \Kf_i\bigg)^{-1}\sum_{i \in \mathcal{I}_{F,n}} \text{Var} \left(\sum_{j=1}^n s_i^{-1} \ex_{\zeta}\big\{\log \tilde m^g(\hat W_{ikj}(\zeta);u_i,v_{ik},\hat \sigma)\big\}\cdot1\{j \in S_i\}\right)$$
Now, let's define $ \mathcal{A}_i=\sum_{j=1}^n s_i^{-1} f(v_iZ_j(\hat \beta, \hat \sigma);u_i,v_{ik}, \hat \sigma)\cdot1\{j \in S_i\}.$ Using independence of the sum, 
$$ \text{Var} (\mathcal{A}_i) \leq \left(\sum_{j=1}^n s_i^{-2}\cdot1\{j \in S_i\}\right) \times \{\max_{1 \leq j \leq n} \text{Var}(f(v_iZ_j(\hat \beta, \hat \sigma);u_i,v_{ik}, \hat \sigma))\}$$
Note that the second term is $O(1)$. Hence, we obtain the following bound
$$\text{Var}(\hat R_{2,n}^{\,g}) \leq n^{-1}\sum_{i \in \mathcal{I}_{F,n}} \text{Var}(\mathcal{A}_i) = O \left(n^{-1} \sum_{i \in \mathcal{I}_{F,n}} 1/s_i\right) = O \left(\frac{D_n}{n}\right).$$  




\noindent \textbf{Proof of Step 3.} 
By definition, 
$$R_{2,n}^g=\frac{1}{n}\sum_{i =1}^n f(\gamma_i,u_i,v_i),$$
where, 
$$f(\gamma,u,v)=\int \bigg\{\log \int \phi\bigg(\frac{\gamma-a}{\sigma (v^2r^{-1}+u^2)^{-1/2}}+z\bigg)g(a)\,da\bigg\}\,\phi(z)\,dz.$$
We assume that $\bm{\gamma}$ are i.i.d. from $\tilde g$ (this is different from $g$), $\bm{u}, \bm{v}$ are i.i.d. from $p_1$ and $p_2$ respectively. Also, $\bm{\gamma}$, $\bm{u}$, $\bm{v}$ are independent among themselves. 

Next, consider: 
$$\hat R_{2,n}^g(h)=\frac{1}{n}\sum_{i \in \mathcal{I}_{F,n}}^n \sum_{j=1}^{n}s_i^{-1}f(\gamma_j,u_i,v_i)1\{j \in S_i\}.$$
As $\bm{\gamma}$, $\bm{u}$ and $\bm{v}$ are independent, by Tower property of conditional expectation, we have: 
$$\ex \{\hat R_{2,n}^g(h)\} = \ex\{R_{2,n}^g\}=\int f(\gamma, u,v) \tilde g(\gamma) p_1(u) p_2(v) d\gamma du dv.$$
Next, note that 
% $\text{Var}(\dot R_2)=n-^{-1}\text{Var}(f(\gamma,u,v))$. Also,
$$\text{Var}(\hat R_{2,n}^g(h))=\text{Var}(E(\hat R_{2,n}^g(h)|\bm{u},\bm{v}))+\ex(\text{Var}(\hat R_{2,n}^g(h)|\bm{u},\bm{v})).$$
% The first term in the right side above is $\text{Var}(n^{-1}\sum_{i=2}^n \ex\{f(\gamma|u_i,v_i)\})$ which is $O_p(n^{-1})$. The second term is $O_p(n^{-1}D_n^2)$
Following the similar steps to the proof of step 2, we obtain the variance is of $O \left(\frac{D_n}{n}\right)$. This completes step 3 of this proof. 

 We have already assessed the asymptotic order of $D_n$. Lemma~\ref{lem:supporting_lemma1} and Lemma~\ref{lem:supporting_lemma2} in conjunction with the 3 steps proved above, conclude Theorem~\ref{thm.risk.conv}.

\begin{lemma}\label{lem:supporting_lemma1}
Let $\{U_i\}_{i\ge1}$ and $\{V_i\}_{i\ge1}$ be independent sequences of i.i.d.\ random variables such that
\[
U_i \sim F_1,\qquad V_i \sim F_2,
\]
and both $F_1$ and $F_2$ have support contained in $[0,M]$ for some fixed $M>0$.
For each $n\in\mathbb{N}$ and $i=1,\dots,n$, define
\[
s_i := \#\{1\le j\le n : U_j \ge U_i + V_i\},
\qquad
D_n := \sum_{i=1}^n \frac{\mathbf{1}_{\{s_i>0\}}}{s_i}.
\]
\[
\mathbb{E}[D_n]
=
\mathbb{E}\!\left[\sum_{i=1}^n \frac{\mathbf{1}_{\{s_i>0\}}}{s_i}\right]
= O(\log n)
\quad\text{as } n\to\infty.
\]
In particular, $D_n = O_p(\log n)$.
\end{lemma}



\noindent \textbf{Proof:} We need assumption (A4) to the prove the above lemma. (A4) implies, there exist constants $\delta>0$ and $c_0>0$ such that, for all $x\in[0,\delta]$,
\[
\mathbb{P}(U_1 \ge M - x)
=
1 - F_1(M-x)
\;\ge\;
c_0 x.
\]
Equivalently, the upper tail of $U_1$ at the right endpoint $M$ is at least linear in the distance to $M$.
Note that this is not too restrictive assumption. Since most of $U, V$ will be truncated at $M$, \[
\int_{M-\delta}^M f_U(x)\,\, dx \geq (M- (M-\delta)) \inf_{x\in(M-\delta,M]} f_U(x) \,\,  = c_0 \delta
\]
Hence, we only need $\inf_{x\in(M-\delta,M]} f_U(x) \neq 0$, which is usually true for most of the distributions unless the the tail probability is slower than a linear rate.

Fix $n$ and $i\in\{1,\dots,n\}$, and set
\[
T_i := U_i + V_i,
\qquad
p_i := \mathbb{P}(U_j \ge T_i \mid T_i)
= 1 - F_1(T_i).
\]
For $j=1,\dots,n$ and $j \neq i$, define $I_{ij} := \mathbf{1}_{\{U_j \ge T_i\}}$. Conditional on $T_i$,
the indicators $\{I_{ij}\}_{j\neq i}$ are i.i.d.\ Bernoulli$(p_i)$, so
\[
s_i \,\big|\, T_i \sim \mathrm{Binomial}(n-1,p_i).
\]
Note that if $T_i>M$ then $p_i=0$ and $s_i=0$ almost surely, so
$\mathbf{1}_{\{s_i>0\}}/s_i = 0$ on $\{T_i>M\}$.

\medskip
\noindent
Now, note that, if $S\sim\mathrm{Binomial}(m,p)$ with $m\ge1$ and $p\in(0,1]$. Then
\[
\frac{\mathbf{1}_{\{S>0\}}}{S} \le \frac{2}{S+1},
\]
hence,
\[
\mathbb{E}\!\left[\frac{\mathbf{1}_{\{S>0\}}}{S}\right]
\le 2\,\mathbb{E}\!\left[\frac{1}{S+1}\right].
\]
We compute
\[
\mathbb{E}\Big[\frac{1}{S+1}\Big]
= \sum_{k=0}^n \frac{1}{k+1}\binom{m}{k} p^k (1-p)^{m-k}.
\]
Using $\frac{1}{k+1}\binom{m}{k} = \frac{1}{m+1}\binom{m+1}{k+1}$,
\[
\mathbb{E}\Big[\frac{1}{S+1}\Big]
= \frac{1}{m+1}
\sum_{k=0}^m \binom{m+1}{k+1} p^k (1-p)^{m-k}
= \frac{1}{(m+1)p}
\sum_{j=1}^{m+1} \binom{m+1}{j} p^j (1-p)^{(m+1)-j}.
\]
The sum equals $1 - (1-p)^{m+1}$, so
\[
\mathbb{E}\Big[\frac{1}{S+1}\Big]
= \frac{1 - (1-p)^{m+1}}{(m+1)p}
\le \frac{1}{(m+1)p}.
\]
Thus, for $p\in(0,1]$,
\begin{equation}\label{eq:binom-bound}
\mathbb{E}\!\left[\frac{\mathbf{1}_{\{S>0\}}}{S}\right]
\le \frac{2}{(m+1)p}
\le 2\min\!\left\{1,\frac{1}{(m+1)p}\right\}.
\end{equation}
For $p=0$ we have $S=0$ almost surely and hence
$\mathbb{E}\big[\mathbf{1}_{\{S>0\}}/S\big]=0$, so
\eqref{eq:binom-bound} trivially holds if we interpret the right-hand side
as $2$.

\noindent Applying this with $S=s_i\mid p_i$, we obtain
\[
\mathbb{E}\!\left[\frac{\mathbf{1}_{\{s_i>0\}}}{s_i} \,\Big|\, p_i\right]
\le 2\min\!\left\{1,\frac{1}{n p_i}\right\},
\]
and hence,
\begin{equation}\label{eq:Ei-bound}
\mathbb{E}\!\left[\frac{\mathbf{1}_{\{s_i>0\}}}{s_i}\right]
\le
2\,\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n p_i}\right\}\right],
\end{equation}
where the integrand is interpreted as $0$ when $p_i=0$.

\noindent By symmetry, the distribution of $p_i$ does not depend on $i$, so let
$p_1$ denote a generic copy. Then
\[
\mathbb{E}[D_n]
=
\sum_{i=1}^n \mathbb{E}\!\left[\frac{\mathbf{1}_{\{s_i>0\}}}{s_i}\right]
\le
2n\,\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n p_1}\right\}\right].
\]

\medskip
\noindent
Now, define
\[
T_1 := U_1 + V_1,\,\, p(t) := \mathbb{P}(U_1 \ge t) = 1 - F_1(t), \qquad t\in[0,M],
\]
so that $p_1 = p(T_1)$.
By (A4), for $x\in[0,\delta]$,
\[
p(M-x) = \mathbb{P}(U_1 \ge M-x) \ge c_0 x.
\]
Define $p_* := p(M-\delta) = \mathbb{P}(U_1 \ge M-\delta)>0$.

\noindent If $T_1 \le M-\delta$, then $p_1 = p(T_1) \ge p_*$ and thus cannot be arbitrarily small. On the other hand, if $T_1\in(M-\delta,M]$, write $T_1=M-x$ with $x\in(0,\delta]$, so that
\[
p_1 = p(M-x) \ge c_0 x,\qquad \text{hence}\quad
p_1 \le y \ \Rightarrow\ x \le y/c_0,\ \ T_1 \ge M - y/c_0.
\]

\noindent Also note that $p_1>0$ implies $T_1\le M$, because $U_1\le M$ almost surely.
Therefore, for any $y>0$,
\[
\{0 < p_1 \le y\} \subseteq \{M - y/c_0 \le T_1 \le M\}.
\]

\noindent  Moreover, for $y>0$ small enough so that $y/c_0 \le \delta$,
\[
\mathbb{P}(0 < p_1 \le y)
\le \mathbb{P}(M - y/c_0 \le T_1 \le M)
= \int_{M-y/c_0}^{M} f_T(t)\,dt
\le C_T \frac{y}{c_0}.
\]
where $C_T =\text{sup}_{t\in [M-y/c_0, M]} \,\,f_T(t)$. Thus there exists $y_0>0$ and a constant $K>0$ such that, for all $0<y\le y_0$,
\begin{equation}\label{eq:small-p}
F_P(y) := \mathbb{P}(0 < p_1 \le y) \le K y.
\end{equation}
\noindent For $n$ large enough we have $1/n \le y_0$.
We do the following split
\[
\min\!\left\{1,\frac{1}{n p_1}\right\}
=
\mathbf{1}_{\{0<p_1 < 1/n\}}
+ \frac{1}{n p_1}\,\mathbf{1}_{\{p_1 \ge 1/n\}}.
\]
Hence,
\[
\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n p_1}\right\}\right]
\le
\mathbb{P}\!\left(0<p_1 < \frac{1}{n}\right)
+ \frac{1}{n}\,\mathbb{E}\!\left[\frac{1}{p_1}\,\mathbf{1}_{\{p_1 \ge 1/n\}}\right].
\]

\noindent Using \eqref{eq:small-p},
\[
\mathbb{P}\!\left(0<p_1 < \frac{1}{n}\right)
\le K\cdot \frac{1}{n}
= O\!\left(\frac{1}{n}\right).
\]

\noindent For the second term, define the cdf $F_P$ of $p_1$ on $(0,1]$ as above.
Then,
\[
\mathbb{E}\!\left[\frac{1}{p_1}\,\mathbf{1}_{\{p_1 \ge 1/n\}}\right]
= \int_{(1/n,1]} \frac{1}{p}\,dF_P(p).
\]
By integration by parts,
\[
\int_{1/n}^1 \frac{1}{p}\,dF_P(p)
= \left[\frac{F_P(p)}{p}\right]_{p=1/n}^{1}
+ \int_{1/n}^1 \frac{F_P(p)}{p^2}\,dp.
\]
Since $F_P(1)\le 1$ and $F_P(1/n)\le K(1/n)$, we have,
\[
\left[\frac{F_P(p)}{p}\right]_{p=1/n}^{1}
\le 1 + K.
\]

\noindent For the integral, split at some fixed $\delta'\in(0,1]$ with $\delta'\le y_0$:
\[
\int_{a/n}^1 \frac{F_P(p)}{p^2}\,dp
= \int_{a/n}^{\delta'} \frac{F_P(p)}{p^2}\,dp
+ \int_{\delta'}^{1} \frac{F_P(p)}{p^2}\,dp.
\]
For $p\in[1/n,\delta']$, \eqref{eq:small-p} gives $F_P(p)\le Kp$, hence
\[
\int_{1/n}^{\delta'} \frac{F_P(p)}{p^2}\,dp
\le K\int_{1/n}^{\delta'} \frac{1}{p}\,dp
= K\log\!\left(\delta' n\right)
= K\log n + O(1).
\]
For $p\in[\delta',1]$, we simply use $F_P(p)\le 1$:
\[
\int_{\delta'}^{1} \frac{F_P(p)}{p^2}\,dp
\le \int_{\delta'}^{1} \frac{1}{p^2}\,dp
= \frac{1}{\delta'} - 1
= O(1).
\]

\noindent Combining these,
\[
\mathbb{E}\!\left[\frac{1}{p_1}\,\mathbf{1}_{\{p_1 \ge 1/n\}}\right]
= O(1+\log n).
\]
Therefore,
\[
\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n p_1}\right\}\right]
\le
O\!\left(\frac{1}{n}\right)
+ \frac{1}{n}\,O(1+\log n)
= O\!\left(\frac{\log n}{n}\right).
\]


\noindent Returning to \eqref{eq:Ei-bound}, we obtain
\[
\mathbb{E}\!\left[\frac{\mathbf{1}_{\{s_i>0\}}}{s_i}\right]
\le 2\,\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n p_i}\right\}\right]
= O\!\left(\frac{\log n}{n}\right),
\]
and by symmetry this bound is the same for each $i=1,\dots,n$. Hence,
\[
\mathbb{E}[D_n]
= \sum_{i=1}^n \mathbb{E}\!\left[\frac{\mathbf{1}_{\{s_i>0\}}}{s_i}\right]
= n \cdot O\!\left(\frac{\log n}{n}\right)
= O(\log n).
\]

\noindent Finally, by Markov's inequality,
$\frac{D_n}{\log n}$ is bounded in probability, i.e. $D_n = O_p(\log n)$.

\noindent This completes the proof.
\begin{lemma}\label{lem:supporting_lemma2}
Let $\{e_i\}_{i\ge1}$ and $\{f_i\}_{i\ge1}$ be independent sequences of i.i.d.\ random variables such that
\[
e_i \sim F_1,\qquad f_i \sim F_2,
\]
and $F_1, F_2$ have support contained in $[0,M]$ for some fixed $M>0$.
Let $\{\xi_i\}_{i\ge1}$ be i.i.d.\ Bernoulli $(\eta_n)$ variables, independent of $(e_i)$ and $(f_i)$, with $\eta_n \in (0,1)$.

\noindent For each $i\ge1$, define
\[
U_i
=
\begin{cases}
e_i, & \xi_i = 0,\\[3pt]
\sum_{j\geq 2} e_{ij}, & \xi_i = 1,
\end{cases}
V_i := f_i,
\]
where $e_{i1},e_{i2}$ are i.i.d.\ copies of $e_i$ (all families independent of each other).
Then $U_i$ has support contained in $[0,sM]$ for some $s\geq 2$ and $V_i$ has support in $[0,M]$.
\[
\mathbb{E}[D_n]
=
\mathbb{E}\!\left[\sum_{i=1}^n \frac{\mathbf{1}_{\{s_i>0\}}}{s_i}\right]
= O(\eta_n^{-1}\log n)
\quad\text{as } n\to\infty.
\]
In particular, $D_n = O_p(\eta_n^{-1}\log n)$.
\end{lemma}
\begin{proof}
Recall, $\mathcal{I}_{F,n}$  denotes the set of units where we can
provide a better shrunken risk estimate. $s_i$ denotes the cardinality of $S_i$,
Define
\[
p_{1i} \;=\; \mathbb{P}\bigl(U > U_i + V_i\bigr),
\qquad
p_{2i} \;=\; \mathbb{P}\bigl(W > U_i + V_i\bigr),
\]
where $W$ is the sum of two independent copies of $U_i$.
We are interested in
\[
\mathbb{E}\left[\sum_{i=1}^n \frac{1}{s_i}\,\mathbf{1}\{i \in \mathcal{I}_{F,n}\}\right].
\]

\noindent Note that $i \notin S_i$ and for all $i \in \mathcal{I}_{F,n}$,
\[
s_i \sim \mathrm{Bin}\bigl(n\eta_n, p_{2i}\bigr)
      + \mathrm{Bin}\bigl(n(1-\eta_n)-1, p_{1i}\bigr)
\;\;\Rightarrow\;\;
s_i \;\ge\; \mathrm{Bin}\bigl(n\eta_n, p_{2i}\bigr).
\]
Next,
\[
\mathbb{E}\!\left[\frac{1}{s_i}\,\Big|\,p_{2i}\right]
\;\le\;
\mathbb{E}\!\left[\frac{1}{n\eta_n p_{2i}}\right].
\]
Hence,
\[
\mathbb{E}\left[\sum_{i=1}^n \frac{1}{s_i}\,\mathbf{1}\{i \in \mathcal{I}_{F,n}\}\,\Big|\,p_{2i}\right]
\;\le\;
n(1-\eta_n)\,
\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n\eta_n p_{2i}}\right\}\right].
\]
Following a similar argument as in Lemma~\ref{lem:supporting_lemma1}, we conclude
\[
\mathbb{E}\!\left[\min\!\left\{1,\frac{1}{n\eta_n p_{2i}}\right\}\right]
= O\!\left(\frac{\log n}{n\eta_n}\right).
\]
Therefore, we can conclude
\[
\mathbb{E} [D_n]
= \mathbb{E}\!\left[\sum_{i \in \mathcal{I}_{F,n}} \frac{1}{s_i}\right]
= O\!\left(\frac{(1 - \eta_n)\log n}{\eta_n}\right) = O\!\left(\frac{\log n}{\eta_n}\right).
\]
Now, note that if $\eta_n = n^{-\beta}$, this implies
\[
\mathbb{E} [D_n] = O\!\left(n^{\beta}\log n\right).
\]
This concludes the lemma.



\end{proof}




==> conference-abstract.tex <==
% %%% You have to change the name of the current file using your name.
% %%% So if you are J. Lember, please name it as "lember.tex" 
% %%% To compile this file, please use the file named "compile_this.tex".

% %% Title of the presentation
% \documentclass[a4paper]{article}

% \def\title#1{{\Large\normalfont \bfseries  \begin{center} #1 \vspace{3pt} \end{center}  } }
% \def\authors#1{{\large\normalfont \bfseries \begin{center} #1 \vspace{1pt} \end{center} } }
% \def\university#1{{\normalfont \slshape \begin{center} #1 \vspace{5pt} \end{center} } }
% \def\inst#1{\vspace{1pt} \unskip$^{#1}$}

% \usepackage{amsthm,mathrsfs,amsfonts,dsfont}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{makeidx}
% \usepackage{enumerate}
% \usepackage{verbatim}
% \usepackage[centering, height=700pt, width = 440pt]{geometry}

% \begin{document}

% \title{Predictive Inference in Linear Mixed Models}
% %% Authors, their affiliation and e-mail
% \authors{Abir Sarkar\inst{1}, Ishan Sengupta\inst{2}, Gourab Mukherjee,\inst{3} and Keisuke Yano\inst{4}}
%  \university{\inst{1} Capital One, India, abir.sarkar@capitalone.com \\
%  \inst{2} Rutgers University, is568@stat.rutgers.edu\\
%  \inst{3} University of Southern California, USA, gourab@usc.edu\\
%  \inst{4} The Institute of Statistical Mathematics, Japan, yano@ism.ac.jp}
% %% Authors' family names for the abstract index
% \index{Lember}
% \index{Matzinger}

% \smallskip

% %% keywords
% \noindent \textbf{Keywords}: Empirical Bayes; Kullback-Leibler loss; Predictive density estimation; Oracle optimality; Shrinkage; Risk estimation; Predictive inference; Linear Mixed Models. 
% \bigskip
% %% Abstract of the presentation

% %% Please insert the abstract of your talk avoiding \newcommand definitions and figures.
% %% Equations should be presented using \begin{equation*} and  \end{equation*}.
% %% Abstract can include references with \cite{key}.
% %% Maximum length of your abstract is one page.


% % We consider predictive inference in \textit{Linear Mixed Models} (LMMs) and study the problem of estimating the predictive density under Kullback-Leibler (KL) loss in LMMs with large number of units. We consider flexible classes of empirical Bayes (EB) predictive densities and develop a novel risk estimation based methodology for selecting hyper-parameters of EB predictive density estimates. Our risk estimation based hyper-parameter selection methodology uses the decision-theoretic identity in Lemma 2 of \cite{george2006improved} that connects predictive KL risk for density estimation to Stein's unbiased estimate of the quadratic risk in point estimation. Direct construction of unbiased KL risk estimates is not possible in LMMs. We leverage information in the covariates and exchangeability of the individual effects to construct asymptotically efficient estimates of the KL risks for wide classes of predictive density estimators. We derive the rates of convergences of the proposed KL risk estimates (KLRE) and show that EB predictors calibrated by minimizing KLREs are asymptotically optimal in LMMs.

% %% References of the abstract
% %% If you have references, include them as follows.
% %% Do not send your .bib file!
% %% If you don't have any references please delete the next lines.

% \begin{thebibliography}{1}
% % journal article
% \bibitem{george2006improved}
% George, E., Liang, F., Xu, X. (2006). Improved minimax predictive densities under {K}ullback--{L}eibler loss. \textit{The Annals of Statistics} 78-91.
% \end{thebibliography}

% \end{document}
